Safe Learning Reference Governor: Theory and Application to Fuel Truck Rollover Avoidance

This paper proposes a learning reference governor (LRG) approach to enforce state and control constraints in systems for which an accurate model is unavailable, and this approach enables the reference governor to gradually improve command tracking performance through learning while enforcing the constraints during learning and after learning is completed. The learning can be performed either on a black-box type model of the system or directly on the hardware. After introducing the LRG algorithm and outlining its theoretical properties, this paper investigates LRG application to fuel truck (tank truck) rollover avoidance. Through simulations based on a fuel truck model that accounts for liquid fuel sloshing effects, we show that the proposed LRG can effectively protect fuel trucks from rollover accidents under various operating conditions.

==> sections/backup_intro.tex <==
Advanced ground vehicles and propulsion systems may operate in various environments, and the performance of these systems is affected by manufacturing variability, aging, degradation and damage. At the same time, safety is considered as a critical factor in these systems, where safety can be represented by constraint satisfactions. These constraints may include but not limited to thermal, power, traction, actuator range/rate, comfort and rollover limits, as well as obstacle avoidance requirements. However, due to changes in environmental factors and component conditions, the system dynamics are often uncertain, and it is hard to know ahead of time what kind of maneuvers may cause constraint violations.

To address such challenges, learning-based approaches have been pursued. For instance, reinforcement learning (RL) has been shown to be a powerful tool to obtain optimal control policies in terms of a pre-specified cost function by exploring system responses under different control signals \cite{sutton2018reinforcement}, \cite{duan2016benchmarking}. RL tries to maximize the long term reward given by the pre-specified cost function by repeatedly observing the system state and taking actions. However, traditional RL algorithms do not address state/output constraints, and it is likely to explore in the unsafe region. Although constraint satisfactions may be promoted through imposing penalties for constraint violations to the cost function, such an approach does not provide an explicit guarantee on constraint enforcement \cite{garcia2015comprehensive}. Other types of safe RL such as constrained policy optimization \cite{achiam2017constrained}, \cite{wachi2018safe} only guarantee near-constraint satisfaction after sufficiently informative learning. Moreover, these safe RL algorithms do not ensure constraint satisfaction during the learning process. As a result, the learning cannot be done on safety-critical hardware systems, where constraint violations may lead to catastrophic consequences. Recently, various safe RL approaches have been proposed, aiming at ensuring constraint satisfaction during learning. These approaches are typically either model-based  \cite{berkenkamp2017safe} or require nominal dynamics of the system to provide a robust controller \cite{cheng2019end}.

Robust model predictive control (MPC) is one approach that optimizes the state trajectories over a receding horizon and guarantees safety by incorporating the disturbances and uncertainties \cite{mayne2005robust}. However, robust MPC relies on a nominal model of the system and oftentimes result in conservative performance. Learning-based MPC integrates model-based control with learning functionality. Theoretical guarantees of learning-based MPC on safety enforcement has been developed in \cite{Aswani_Gonzalez_LearningMPC}. However, a nominal linear model and bound on deviations of the system dynamics are required. Specifically, learning-based MPC algorithms typically pursue to learn/estimate a model that can represent the system dynamics under the current operating condition, and then use this learned/estimated model to compute control signals \cite{Robust_cons_LNMPC}. Meanwhile, Gaussian Process (GP) has been employed in many learning-based MPC works \cite{Gaussian_MPC}, \cite{LMPC_safe_explor}. Although good performance is achieved, theoretical guarantee on safety is missing from these approaches. 

Iterative learning control (ILC) is another technique that learns from previous experience to improve the controller performance \cite{bristow2006survey}. However, the focus of ILC is oftentimes on improving the performance over a single and repeated operation \cite{norrlof2002adaptive}. There has been applications of ILC to systems without identical operations \cite{kawamura2002analysis}, but similar motions is observed in different tasks and these motions are related by a time-scale transformation. 

Reference Governor (RG) is an add-on scheme to a nominal closed-loop system, acting as a pre-filter to modify set-point commands to the nominal system to guard the system against potential constraint violations \cite{Garone_Survey}. Such an add-on scheme is ideal for integration with the legacy systems as it does not need to change the existing/legacy controllers. In \cite{Kaiwen_Model_Free_Learning}, a model-free learning-based approach to enforcing state/output constraints based on a reference governor scheme has been proposed for non safety-critical control systems, where constraint violations are undesirable but do not lead to catastrophic consequences. The learning algorithm proposed in \cite{Kaiwen_Model_Free_Learning} evolves the reference governor parametrization based on observed constraint violations during the learning phase and gradually eliminates them over time.

With respect to the existing approaches, the method proposed in present paper is distinguished by its model-free characteristics with minimal knowledge requirement of the system and safety guarantee during and after learning. The proposed approach has the following advantages: a) the proposed approach is based on reference governor, which is an add-on scheme to the legacy system, and as a result, it is suitable for systems that already has a well-performed nominal controller but additional safety requirements are imposed; b) the proposed approach is a model-free approach with minimal knowledge of the system, and the required information can be obtained by running a series of experiments before learning; c) safety or constraint enforcement is guaranteed theoretically both during and after learning, and as a result, the approach can be applied to some safety-critical control systems, where constraint violations can lead to catastrophic consequences; d) the safety guarantee does not rely on the length of the learning; in other words, the proposed approach is able to ensure safety for any amount of training time, but the longer training time it takes, the more aggressive behavior it is able to achieve. Specifically, we propose a novel learning-based approach based on a reference governor scheme, to operating a control system where any constraint violation is not allowed. The reference governor starts from a conservative design and the learning algorithm evolves the reference governor parametrization to gradually improve its performance in terms of response speed while guaranteeing constraint satisfaction for all time, both during and after the learning phase. Also, the learning algorithm does not rely on an explicit model of the control system.

Tank trucks have been widely used in transporting chemical and petroleum products. However, accidents associated with these tank trucks may also lead to severe people injury and huge property damage. According to \cite{treichel2006safety}, rollover is the most frequent accidents associated with the tank trucks. Since these trucks are partially filled most of the time, researchers concluded that liquid sloshing is the main cause to the rollover accidents \cite{salem1999review}, \cite{kang2002cargo}. Based on these studies, the free space in the partially-filled tank allows liquid sloshing to happen when the vehicle state changes, and truck's driving stability is severely affected due to the sloshing force. Fuel sloshing models have been investigated to further analyze its influence on tank truck. Many previous research has been limited to quasi-static models due to the computational complexity associated with the fluid dynamics \cite{modaressi2007three}. However, the sloshing force and torque caused by transient liquid sloshing cannot be captured by the quasi-static model. An equivalent mechanical model has been developed to model the transient behavior of lateral liquid sloshing \cite{slosh_model}, \cite{equiv_model}, where the model is validated based on high-fidelity FLUENT simulations. 

To illustrate the algorithm functionality and characteristics, we consider a simulation study of fuel truck rollover avoidance under sloshing effect. An equivalent mechanical model for lateral fuel sloshing is first described, and vehicle dynamics is integrated with the lateral sloshing model for the simulation study. The fuel truck model is validated against the high-fidelity FLUENT results presented in \cite{slosh_model}. The proposed learning reference governor approach is then applied to the fuel truck model. Results during learning process, step response results and sine-and-dwell test results are reported, where safety is enforced both during and after learning, and as learning progresses, the proposed approach is able to push the system towards the boundary of the constraint without crossing it.

The contribution of the paper is summarized as follows: a) we develop a novel learning approach based on the reference governor framework to enforce safety with minimal requirements on system knowledge; b) theoretical guarantees on constraint enforcement both during and after learning have been established; c) the lateral driving stability of fuel trucks is investigated based on an equivalent lateral sloshing model; d) we demonstrate that the proposed approach can be applied to fuel truck rollover avoidance based on an equivalent lateral sloshing model. %e) the proposed approach can be extended to handle driving condition changes (such as speed, load, bank angle etc).

The paper is organized as follows. In Section~\ref{sec:problem_formulation}, we formulate the problem considered in this paper. In Section~\ref{sec:learning_rg}, we present the safety-enforced learning reference governor algorithm we proposed along with its theoretical properties and associated proofs. Section~\ref{sec:truck_dyn} describes the equivalent mechanical model of fuel sloshing as well as the vehicle dynamics model. Section~\ref{sec:results} illustrates the simulation results obtained from the fuel tank model and learning reference governor. Finally, the summary of the current work and envisioned future work is included in Section~\ref{sec:conclusion}.

The notations used in this paper are standard. In particular, for a right-continuous signal $\theta:[0,\infty) \to \Theta$, we use $\theta(t^-)$ to denote the left-sided limit $\lim_{t' \nearrow t} \theta(t')$, and for a better distinction, we also use $\theta(t^+)$ to denote $\theta(t)$.
